VSLAM-LAB: A Comprehensive Framework for Visual SLAM Methods and Datasets

Visual Simultaneous Localization and Mapping (VSLAM) research faces significant challenges due to fragmented toolchains, complex system configurations, and inconsistent evaluation methodologies. To address these issues, we present VSLAM-LAB, a unified framework designed to streamline the development, evaluation, and deployment of VSLAM systems. VSLAM-LAB simplifies the entire workflow by enabling seamless compilation and configuration of VSLAM algorithms, automated dataset downloading and preprocessing, and standardized experiment design, execution, and evaluation--all accessible through a single command-line interface. The framework supports a wide range of VSLAM systems and datasets, offering broad compatibility and extendability while promoting reproducibility through consistent evaluation metrics and analysis tools. By reducing implementation complexity and minimizing configuration overhead, VSLAM-LAB empowers researchers to focus on advancing VSLAM methodologies and accelerates progress toward scalable, real-world solutions. We demonstrate the ease with which user-relevant benchmarks can be created: here, we introduce difficulty-level-based categories, but one could envision environment-specific or condition-specific categories.

==> 04_vslam.tex <==
\section{Visual SLAM}

\subsection{Evaluation}
\textbf{Absolute Trajectory Error (ATE)} \cite{sturm12iros}


==> figure_config_difficult.tex <==
\begin{figure}[t]
\centering
\resizebox{\linewidth}{!}{ % 
\begin{tabular}{C{0.15\linewidth}C{0.15\linewidth}C{0.15\linewidth}C{0.15\linewidth}C{0.15\linewidth}C{0.15\linewidth}}
\arrayrulecolor{vslamlab}
\footnotesize TUM-RGBD& \footnotesize TUM-RGBD & \footnotesize ETH3D & \footnotesize HILTI  &  \footnotesize EUROC \\
\footnotesize Fr1. Desk2& \footnotesize Fr.3 n.n.f. & \footnotesize L. Loop 1 & \footnotesize Exp 04 &  \footnotesize MH04 Dif. \\
\hline
\\
\multicolumn{5}{c}{\includegraphics[width=1\linewidth]{figures/config_difficult/canvas_sequences.png}} \\
\multicolumn{5}{c}{\includegraphics[width=1\linewidth]{figures/config_difficult/trajectories.pdf}} \\
\multicolumn{5}{c}{\includegraphics[width=1\linewidth]{figures/config_difficult/accuracy_boxplot_detailed.pdf}} \\
\end{tabular}
}
\resizebox{0.75\linewidth}{!}{
\begin{tabular}{ccccc}
\myline{mast3r} MASt3R-SLAM & \myline{droid} DROID-SLAM
\end{tabular}
}
\caption{\textbf{Difficult 2025.}}
\label{fig:configDifficult}
\end{figure}

==> figure_config_easy.tex <==
\begin{figure}[t]
\centering
\resizebox{\linewidth}{!}{ % 
\begin{tabular}{C{0.15\linewidth}C{0.15\linewidth}C{0.15\linewidth}C{0.15\linewidth}C{0.15\linewidth}C{0.15\linewidth}}
\arrayrulecolor{vslamlab}
\footnotesize RGBDTUM& \footnotesize ETH3D & \footnotesize 7SCENES & \footnotesize EUROC  &  \footnotesize KITTI \\
\footnotesize Fr.3 s.t.f & \footnotesize Table 3 & \footnotesize Chess 01 & \footnotesize V1 01 E.&  \footnotesize KITTI 04 \\
\hline
\\
\multicolumn{5}{c}{\includegraphics[width=1\linewidth]{figures/config_easy/canvas_sequences.png}} \\
\multicolumn{5}{c}{\includegraphics[width=1\linewidth]{figures/config_easy/trajectories.pdf}} \\
\multicolumn{5}{c}{\includegraphics[width=1\linewidth]{figures/config_easy/accuracy_boxplot_detailed.pdf}} \\
\end{tabular}
}
\resizebox{1\linewidth}{!}{
\begin{tabular}{ccccc}
\myline{mast3r} MASt3R-SLAM & \myline{droid} DROID-SLAM & \myline{dpvo} DPVO & \myline{orbslam} ORB-SLAM2
\end{tabular}
}
\caption{\textbf{Easy 2025.} The top row shows RGB frames from the sequences, the middle row illustrates the camera trajectories, and the bottom row presents boxplots of ATE for the estimated trajectories.}
\label{fig:configEasy}
\end{figure}

==> figure_config_extreme.tex <==
\begin{figure}[t]
\centering
\resizebox{\linewidth}{!}{ % 
\begin{tabular}{C{0.15\linewidth}C{0.15\linewidth}C{0.15\linewidth}C{0.15\linewidth}C{0.15\linewidth}C{0.15\linewidth}}
\arrayrulecolor{vslamlab}
\footnotesize RGBDTUM& \footnotesize ETH3D & \footnotesize ETH3D & \footnotesize OPENLORIS  &  \footnotesize DRUNKARDS \\
\footnotesize Fr.3 Walk & \footnotesize Ceiling 2 & \footnotesize Einstein G. & \footnotesize Cafe 1 &  \footnotesize 00000 \\
\hline
\\
\multicolumn{5}{c}{\includegraphics[width=1\linewidth]{figures/config_extreme/canvas_sequences.png}} \\
\multicolumn{5}{c}{\includegraphics[width=1\linewidth]{figures/config_extreme/trajectories.pdf}} \\
\multicolumn{5}{c}{\includegraphics[width=1\linewidth]{figures/config_extreme/accuracy_boxplot_detailed.pdf}} \\
\end{tabular}
}
\resizebox{0.75\linewidth}{!}{
\begin{tabular}{ccccc}
\myline{mast3r} MASt3R-SLAM & \myline{droid} DROID-SLAM
\end{tabular}
}
\caption{\textbf{Extreme 2025.}}
\label{fig:configExtreme}
\end{figure}

==> figure_config_medium.tex <==
\begin{figure}[t]
\centering
\resizebox{\linewidth}{!}{ % 
\begin{tabular}{C{0.15\linewidth}C{0.15\linewidth}C{0.15\linewidth}C{0.15\linewidth}C{0.15\linewidth}C{0.15\linewidth}}
\arrayrulecolor{vslamlab}
\footnotesize REPLICA& \footnotesize ICLNUIM & \footnotesize SCANNET++ & \footnotesize RGBDTUM  &  \footnotesize TARTANAIR \\
\footnotesize Office 0 & \footnotesize l.r. traj0 & \footnotesize Scannet 56 & \footnotesize Fr.3 nsnt f. &  \footnotesize ME001 \\
\hline
\\
\multicolumn{5}{c}{\includegraphics[width=1\linewidth]{figures/config_medium/canvas_sequences.png}} \\
\multicolumn{5}{c}{\includegraphics[width=1\linewidth]{figures/config_medium/trajectories.pdf}} \\
\multicolumn{5}{c}{\includegraphics[width=1\linewidth]{figures/config_medium/accuracy_boxplot_detailed.pdf}} \\
\end{tabular}
}
\resizebox{0.75\linewidth}{!}{
\begin{tabular}{ccccc}
\myline{mast3r} MASt3R-SLAM & \myline{droid} DROID-SLAM
\end{tabular}
}
\caption{\textbf{Medium 2025.} The top row shows RGB frames from the sequences, the middle row illustrates the camera trajectories, and the bottom row presents boxplots of ATE for the estimated trajectories.}
\label{fig:configSynthetic}
\end{figure}

==> figure_pipeline.tex <==
\begin{figure}[t]
\centering
\resizebox{\linewidth}{!}{ % 
\begin{tabular}{c}
\includegraphics[width=1\linewidth]{example-image-a} 
\end{tabular}
}
\caption{\textbf{Pipeline.}}
\label{fig:pipeline}
\end{figure}

==> tables/time_config_easy.tex <==
\begin{table}[t]
\centering
% \setlength{\tabcolsep}{5pt} 
% \rowcolors{2}{gray!15}{white} 
\resizebox{1.0\columnwidth}{!}{
\begin{tabular}{lcccc}

 & \textbf{\textcolor[HTML]{FF0000}{DPVO}} & \textbf{\textcolor[HTML]{008000}{DROID-SLAM}} & \textbf{\textcolor[HTML]{FFA500}{MASt3R-SLAM}} & \textbf{\textcolor[HTML]{0000FF}{ORB-SLAM2}} \\
\midrule
V1 01 easy & 51.52 & 75.56 & 59.07 & 54.95 \\
chess 01 & 50.01 & 70.01 & 80.01 & 50.01 \\
fr1 xyz & 55.15 & 137.86 & 87.73 & 50.14 \\
office0 & 60.01 & 55.01 & 55.01 & 45.01 \\
table 3 & 59.33 & 59.33 & 67.81 & 50.86 \\
\bottomrule
\textbf{Overall} & 55.20 $\pm$ 4.97 & 79.55 $\pm$ 30.68 & 69.93 $\pm$ 12.63 & 50.19 $\pm$ 3.23 \\

\end{tabular}
}
\caption{\textbf{VSLAM-LAB Methods}: Visual SLAM \& Multi-view reconstruction methods for monocular cameras contained in VSLAM-LAB.}
\label{tab:pipelines}
\end{table}



